Convergence Analysis of Discrete Conformal Transformation

Continuous conformal transformation minimizes the conformal energy. The convergence of minimizing discrete conformal energy when the discrete mesh size tends to zero is an open problem. This paper addresses this problem via a careful error analysis of the discrete conformal energy. Under a weak condition on triangulation, the discrete function minimizing the discrete conformal energy converges to the continuous conformal mapping as the mesh size tends to zero.

==> head.tex <==
\usepackage[utf8]{inputenc}
\usepackage{amsmath,amssymb,amsthm,bm}
\usepackage{amsfonts}
\usepackage{mathrsfs}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{enumitem}
\usepackage{overpic}
\usepackage{multirow}
\usepackage{nicefrac}
\numberwithin{equation}{section}
\usepackage{subfig}
\usepackage{float}
\usepackage{caption}
\renewcommand{\thefigure}{\arabic{section}-\arabic{figure}}
\renewcommand{\thetable}{\arabic{section}-\arabic{table}}
\usepackage{multicol}
\linespread{1.3}
\usepackage{dsfont}
\usepackage{bbm}
\usepackage{bm}
\usepackage{url}
\usepackage{verbatim}
\usepackage{algorithm,algorithmic}
\usepackage{xcolor}

\usepackage[colorlinks,linkcolor=blue,
            citecolor=blue]{hyperref}
            
\usepackage[
backend=biber,
style=nature,
sorting=ynt
]{biblatex}

\usepackage{geometry}
\geometry{a4paper,left=2.5cm,right=2.5cm,top=2cm,bottom=2cm}

\usepackage{cleveref}
\usepackage{biblatex}
\addbibresource{reference.bib}

\usepackage{slashed}


\newcommand{\x}{\mathbf{x}}
\newcommand{\diff}{\,{\mathrm d}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\tr}{\mathrm{trace}}
\newcommand*\Laplace{\mathop{}\!\mathbin\bigtriangleup}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\trace}{\mathrm{trace}}
\newcommand{\st}{{\rm s.t.}}
\newcommand{\rdot}{{\rm rdot}}
\newcommand{\sgn}{{\rm sgn}}

\newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{observation}{Observation}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{question}{Question}

\providecommand{\keywords}[1]
{
  \small	
  \textbf{\textit{Key words---}} #1
}

\graphicspath{
{images/}
}
